Rate-Distortion via Markov Chain Monte Carlo

We propose an approach to lossy source coding, utilizing ideas from Gibbs sampling, simulated annealing, and Markov Chain Monte Carlo (MCMC). The idea is to sample a reconstruction sequence from a Boltzmann distribution associated with an energy function that incorporates the distortion between the source and reconstruction, the compressibility of the reconstruction, and the point sought on the rate-distortion curve. To sample from this distribution, we use a `heat bath algorithm': Starting from an initial candidate reconstruction (say the original source sequence), at every iteration, an index i is chosen and the i-th sequence component is replaced by drawing from the conditional probability distribution for that component given all the rest. At the end of this process, the encoder conveys the reconstruction to the decoder using universal lossless compression. The complexity of each iteration is independent of the sequence length and only linearly dependent on a certain context parameter (which grows sub-logarithmically with the sequence length). We show that the proposed algorithms achieve optimum rate-distortion performance in the limits of large number of iterations, and sequence length, when employed on any stationary ergodic source. Experimentation shows promising initial results. Employing our lossy compressors on noisy data, with appropriately chosen distortion measure and level, followed by a simple de-randomization operation, results in a family of denoisers that compares favorably (both theoretically and in practice) with other MCMC-based schemes, and with the Discrete Universal Denoiser (DUDE).

==> counts.tex <==
Let $H_k (y^n)$ denote the conditional empirical entropy of order $k$ induced by $y^n$, i.e.~
\begin{equation}\label{eq: emp cond distribution}
    H_k (y^n) = H(Z_{k+1} | Z^{k}) ,
\end{equation}
where $Z^{k+1}$ on the right hand side of (\ref{eq: emp cond
distribution}) is distributed according to
\begin{equation}\label{eq: kponeth empirical distribution}
    P (Z^{k+1} = u^{k+1}) = \frac{1}{n} \left|  \left\{ 1 \leq i \leq n : y_{i-k}^i = u^{k+1}    \right\}
    \right|,
\end{equation}
where in \eqref{eq: kponeth empirical distribution}, and throughout we
assume a cyclic convention whereby $y_i \triangleq y_{n+i}$ for $i
\leq 0$. We introduce the count notation $\mathbf{m} (y^n)$, a matrix of size $|\Yc|\times|\Yc|^{k}$, to denote the $(k+1)^{\rm th}$ order empirical distribution of the sequence $y^n$. More
explicitly, for $\b\in\Yc$ and $\bb=b^k\in{\Yc}^k$, $\mathbf{m}_{\cdot,\bb}(y^n)$ is a column vector whose
$\b^{\rm th}$ component is given by
\begin{equation}\label{eq: m vector defined}
m_{\b,\bb}(y^n) = \frac{1}{n-k} \left| \left\{ k+1 \leq i \leq n :
y_{i-k}^{i-1} = \bb, y_i=\b]    \right\}\right|,
\end{equation}
Note that, with the count notation, the conditional empirical entropy in \eqref{eq: emp cond distribution} can
be expressed as 
\begin{equation}\label{eq: alternative representation of Hk}
H_k (y^n) = \frac{1}{n} \sum_{\bb} \mathcal{H} \left(\mathbf{m}_{\cdot,\bb}(y^n)\right) \mathbf{1}^T \mathbf{m}_{\cdot,\bb}(y^n),
\end{equation}
where $\mathbf{1}$ denotes the all-ones column vector of length
$|\mathcal{Y}|$, and for a vector $\mathbf{v} = (v_1, \ldots , v_\ell)^T$
with non-negative components, we let $\mathcal{H}(\mathbf{v})$ denote the
entropy of the random variable whose probability mass function (pmf)
is proportional to $v$. Formally,
\begin{equation}\label{eq: single letter ent functional defined}
\mathcal{H} (\mathbf{v}) = \left\{ \begin{array}{cc}
                           \sum\limits_{i=1}^\ell \frac{v_i}{\| \mathbf{v}
\|_1}  \log \frac{\| \mathbf{v} \|_1}{v_i} &  \mbox{ if }  \mathbf{v}
\neq (0, \ldots , 0)^T \\
                           0 & \mbox{ if } \mathbf{v}  = (0, \ldots , 0)^T,
                         \end{array}
\right.
\end{equation}
where $0\log(0) = 0$ by convention.

